SyncVIS: Synchronized Video Instance Segmentation

Recent DETR-based methods have advanced the development of Video Instance Segmentation (VIS) through transformers' efficiency and capability in modeling spatial and temporal information. Despite harvesting remarkable progress, existing works follow asynchronous designs, which model video sequences via either video-level queries only or adopting query-sensitive cascade structures, resulting in difficulties when handling complex and challenging video scenarios. In this work, we analyze the cause of this phenomenon and the limitations of the current solutions, and propose to conduct synchronized modeling via a new framework named SyncVIS. Specifically, SyncVIS explicitly introduces video-level query embeddings and designs two key modules to synchronize video-level query with frame-level query embeddings: a synchronized video-frame modeling paradigm and a synchronized embedding optimization strategy. The former attempts to promote the mutual learning of frame- and video-level embeddings with each other and the latter divides large video sequences into small clips for easier optimization. Extensive experimental evaluations are conducted on the challenging YouTube-VIS 2019 & 2021 & 2022, and OVIS benchmarks and SyncVIS achieves state-of-the-art results, which demonstrates the effectiveness and generality of the proposed approach. The code is available at https://github.com/rkzheng99/SyncVIS.

==> tab/Nk_Ts.tex <==
\begin{table}
\centering
\vspace{-5pt}
\caption{Ablation study on the aggregation embedding size $N_{k}$ of synchronized video-frame modeling and the sub-clip size $T_{s}$ of synchronized embedding optimization.}
\scriptsize
\setlength{\tabcolsep}{1mm}{
\begin{tabular}{l|ccccc|c|ccccc@{}}\toprule
$N_{k}$ &AP &AP$_{50}$ &AP$_{75}$ &AR$_{1}$ &AR$_{10}$ &$T_s$ &AP &AP$_{50}$ &AP$_{75}$ &AR$_{1}$ &AR$_{10}$\\\midrule
5  &51.1  &73.0 &55.4 &49.1 &59.3 &1 &50.9 &73.7 &54.9 &49.0 &60.1\\
10 &51.5  &{73.2}    & {55.9}  & {49.5}  &60.4 &2 &51.3  &{73.3}    & {55.6}  & {49.2}  &60.2\\
25 &50.9 &73.5 &55.1 &48.4 &59.6 &3  &51.5  &{73.2}  & {55.9}  & {49.5}  &60.4\\
50 &49.3 &72.8 &52.3 &47.4 &56.7 &4 &50.7 &73.8 &54.1 &47.9 &58.9\\
100 &47.5 &70.4 &51.4 &46.8 &56.1 &5 &50.4 &73.3 &54.2 &47.2 &58.1\\
\bottomrule
\end{tabular}}

\vspace{-10pt}
\label{tab:k&T}
\end{table}

\begin{table}[t]
\centering

\caption{Ablation study on the synchronized embedding optimization strategy with ResNet-50 backbone on multiple datasets.}
\vspace{-5pt}
\scriptsize
\setlength{\tabcolsep}{2.6mm}{
\begin{tabular}{l|l|ccc}\toprule
Datasets &Method  &AP &AP$_{50}$ &AP$_{75}$ \\\midrule
\multirow{2}{*}{YouTube-VIS 2019} &Mask2Former-VIS &46.4 &68.0 &50.0 \\ 
 &\cellcolor[HTML]{efefef}{+ Optimization} &\cellcolor[HTML]{efefef}47.1 &\cellcolor[HTML]{efefef}68.9 &\cellcolor[HTML]{efefef}50.8 \\

\hline
\multirow{2}{*}{YouTube-VIS 2021} &Mask2Former-VIS &40.6 &60.9 &41.8 \\
&\cellcolor[HTML]{efefef}{+ Optimization} &\cellcolor[HTML]{efefef}41.7 &\cellcolor[HTML]{efefef}62.1 &\cellcolor[HTML]{efefef}42.5 \\ \hline
\multirow{2}{*}{OVIS} &Mask2Former-VIS &11.1 &26.0 &7.6 \\
&\cellcolor[HTML]{efefef}{+ Optimization} &\cellcolor[HTML]{efefef}12.3 &\cellcolor[HTML]{efefef}27.1 &\cellcolor[HTML]{efefef}9.2 \\
\bottomrule
\end{tabular}}

\label{tab:optimization}
\vspace{-18pt}
\end{table}

==> tab/combine_fig.tex <==
\begin{figure}[htp]
    \vspace{-10pt}
    \centering
    % \caption{\textbf{Comparison on referring video segmentation and video instance segmentation datasets.} }
    \begin{minipage}{0.45\textwidth}
        
            % \end{footnotesize}
        \centering
        \includegraphics[width=0.95\linewidth]{fig/input.pdf}
        \vspace{-10pt}
        \caption{Ablation study on the complexity of video scenarios regarding the number of input frames $T$.}
        \label{fig:input_length}
    \end{minipage}
    \hfill
    \begin{minipage}{0.48\textwidth}
        \captionof{table}{Ablation study on key component designs in SyncVIS.}
        \label{tab:separate_effect}
        \scriptsize
        \resizebox{\linewidth}{!}
        {
            \begin{tabular}{l|ccc}\toprule
            Method &AP &AP$_{50}$ &AP$_{75}$ \\\midrule
            Mask2Former-VIS~\cite{cheng2021mask2former} &45.1 &65.7 &49.0 \\
            + Synchronized Video-Frame Modeling &50.3 &72.9 &54.1 \\
            + Synchronized Embedding Optimization &46.7 &68.2 &50.3 \\
            \cellcolor[HTML]{efefef}{+ Both (SyncVIS)} &\cellcolor[HTML]{efefef}51.5 &\cellcolor[HTML]{efefef}73.2 &\cellcolor[HTML]{efefef}55.9 \\
            \midrule
            VITA~\cite{heo2022vita} &49.5 &72.1 &54.3 \\
            + Synchronized Video-Frame Modeling &53.0 &74.7 &57.4 \\
            + Synchronized Embedding Optimization &51.2 &73.6 &57.6 \\
            \cellcolor[HTML]{efefef}{+ Both (SyncVIS)} &\cellcolor[HTML]{efefef}54.2 &\cellcolor[HTML]{efefef}75.1 &\cellcolor[HTML]{efefef}58.2 \\
            \bottomrule
            \end{tabular}
        }
    \end{minipage}
\end{figure}

==> tab/main_ablation.tex <==
\begin{table}[htp]
    \vspace{-15pt}
    \centering
    % \caption{\textbf{Comparison on referring video segmentation and video instance segmentation datasets.} }
    \begin{minipage}{0.46\textwidth}
        \captionof{table}{Ablation study on synchronized video-frame modeling.}
        \label{tab:mutual}
        \resizebox{\linewidth}{!}
        {
            % \end{footnotesize}
            \begin{tabular}{l|cc|ccc}\toprule
            ID      &Frame$\rightarrow$Video        &Video$\rightarrow$Frame         &AP  &AP$_{50}$ &AP$_{75}$  \\
            \midrule
            \Rom{1} &           &            &45.1 &65.7 &49.0 \\
            \Rom{2} &\checkmark &            &50.2 &72.5 &54.2 \\
            \Rom{3} &           &\checkmark  &48.6 &71.4 &51.8 \\
            \Rom{4} &\checkmark &\checkmark  &\cellcolor[HTML]{efefef}51.5 &\cellcolor[HTML]{efefef}73.2 &\cellcolor[HTML]{efefef}55.9\\
            
            \bottomrule
            \end{tabular}
        }
    \end{minipage}
    \hfill
    \begin{minipage}{0.5\textwidth}
        \captionof{table}{Ablation study on the structure and query selection of synchronized video-frame modeling.}
        \label{tab:cascade}
        \scriptsize
        \resizebox{\linewidth}{!}
        {
            \begin{tabular}{l|ccc}\toprule
            Method &AP &AP$_{50}$ &AP$_{75}$ \\
            \midrule
            Cascade Structure + Frame-level Queries &46.2 &67.8 &49.9 \\
            Cascade Structure + Video-level Queries &46.7 &68.2 &50.3 \\
            Cascade Structure + Both Queries &49.9 &72.0 &54.4 \\
            \cellcolor[HTML]{efefef}Synchronous Structure + Both Queries (SyncVIS) &\cellcolor[HTML]{efefef}51.5 &\cellcolor[HTML]{efefef}73.2 &\cellcolor[HTML]{efefef}55.9 \\
            \bottomrule
            \end{tabular}
        }
    \end{minipage}
    \vspace{-15pt}
\end{table}

==> tab/vis_ovis.tex <==
\begin{table}[htp]
    \vspace{-10pt}
    \centering
    % \caption{\textbf{Comparison on referring video segmentation and video instance segmentation datasets.} }
    \begin{minipage}{0.46\textwidth}
        \captionof{table}{Comparison on the YouTube-VIS 2022 long videos.}
        \label{tab:ytvis22}
        \resizebox{\linewidth}{!}
        {
            % \end{footnotesize}
            \tablestyle{5pt}{1.02}
            \begin{tabular}{@{}c|l|ccccc}\toprule
            &Method &AP &AP$_{50}$ &AP$_{75}$ &AR$_{1}$ &AR$_{10}$ \\\midrule        
            \multirow{4}{*}{\rotatebox{90}{Swin-L}}
            &VITA~\cite{heo2022vita} &41.1 &63.0 &44.0 &\textbf{39.3} &44.3 \\
            &MinVIS~\cite{huang2022minvis} &33.1 &54.8 &33.7 &29.5 &36.6 \\
            &DVIS~\cite{zhang2023dvis} &45.9 &69.0 &\textbf{48.8} &37.2 &51.8\\
            &\cellcolor{lightgray!30}SyncVIS &\cellcolor{lightgray!30}\textbf{47.0} &\cellcolor{lightgray!30}\textbf{69.4} &\cellcolor{lightgray!30}{48.6}&\cellcolor{lightgray!30}{38.9} &\cellcolor{lightgray!30}\textbf{52.4} \\
            \bottomrule
            \end{tabular}
        }
    \end{minipage}
    \hfill
    \begin{minipage}{0.5\textwidth}
        \captionof{table}{Results comparison on the OVIS validation set.}
        \label{tab:ovis}
        \scriptsize
        \resizebox{\linewidth}{!}
        {
            \tablestyle{5pt}{1.02}
            \begin{tabular}{@{}c|l|ccccc}\toprule
            &Method &AP &AP$_{50}$ &AP$_{75}$ &AR$_{1}$ &AR$_{10}$ \\\midrule        
            \multirow{2}{*}{\rotatebox{90}{R-50}} 

            &DVIS~\cite{zhang2023dvis} &34.1 &59.8 &32.3 &15.9 &41.1 \\
            &\cellcolor{lightgray!30}SyncVIS &\cellcolor{lightgray!30}\textbf{36.3} &\cellcolor{lightgray!30}\textbf{60.9} &\cellcolor{lightgray!30}\textbf{33.0} &\cellcolor{lightgray!30}\textbf{17.0} &\cellcolor{lightgray!30}\textbf{42.8} \\
            \midrule
            \multirow{4}{*}{\rotatebox{90}{Swin-L}}
            &VITA~\cite{heo2022vita} &27.7 &51.9 &24.9 &14.9 &33.0 \\

            &CTVIS~\cite{ying2023ctvis} &46.9 &71.5 &47.5 &19.1 &52.1\\
            &DVIS~\cite{zhang2023dvis} &49.9 &\textbf{75.9} &53.0 &19.4 &55.3 \\
            &\cellcolor{lightgray!30}SyncVIS &\cellcolor{lightgray!30}\textbf{50.8} &\cellcolor{lightgray!30}{75.7} &\cellcolor{lightgray!30}\textbf{53.1}&\cellcolor{lightgray!30}\textbf{20.5} &\cellcolor{lightgray!30}\textbf{55.9} \\
            \bottomrule
            \end{tabular}
        }
    \end{minipage}
\end{table}
